A new twist on modular links from an old perspective

We show that the complement of arithmetic modular links found in arXiv:2307.09409 is homeomorphic to the complement of augmented chainlinks. In particular, these link complements arise as n-fold cyclic covers of the Whitehead link complement.

==> Figures/LR_L2R2.tex <==
\definecolor{linkcolor0}{rgb}{0.85, 0.15, 0.15}
\definecolor{linkcolor1}{rgb}{0.15, 0.15, 0.85}
\definecolor{linkcolor2}{rgb}{0.15, 0.85, 0.15}
\begin{tikzpicture}[line width=1.3, line cap=round, line join=round]
  \begin{scope}[color=linkcolor0]
    \draw (7.89, 2.19) .. controls (8.72, 1.20) and (7.11, 0.11) .. 
          (4.99, 0.09) .. controls (2.83, 0.07) and (0.92, 0.82) .. (1.73, 1.97);
    \draw (1.73, 1.97) .. controls (1.83, 2.11) and (1.93, 2.25) .. (2.03, 2.39);
    \draw (2.03, 2.39) .. controls (2.15, 2.57) and (2.28, 2.75) .. (2.40, 2.92);
    \draw (2.40, 2.92) .. controls (2.52, 3.09) and (2.64, 3.26) .. (2.76, 3.43);
    \draw (2.76, 3.43) .. controls (2.91, 3.65) and (3.07, 3.87) .. (3.22, 4.10);
    \draw (3.34, 4.26) .. controls (3.49, 4.47) and (3.64, 4.68) .. (3.79, 4.90);
    \draw (3.90, 5.06) .. controls (4.01, 5.22) and (4.13, 5.38) .. (4.24, 5.54);
    \draw (4.35, 5.70) .. controls (4.42, 5.80) and (4.49, 5.90) .. (4.56, 6.00);
    \draw (4.68, 6.16) .. controls (5.59, 7.46) and (7.13, 8.28) .. 
          (8.31, 7.46) .. controls (9.89, 6.38) and (8.93, 4.14) .. (7.82, 2.27);
    \draw (7.82, 2.27) .. controls (7.19, 1.20) and (5.83, 1.01) .. 
          (4.56, 1.03) .. controls (3.45, 1.05) and (2.05, 1.08) .. (1.76, 1.88);
    \draw (1.69, 2.06) .. controls (0.97, 4.03) and (0.06, 6.50) .. 
          (1.18, 7.68) .. controls (2.14, 8.71) and (3.51, 7.40) .. (4.62, 6.08);
    \draw (4.62, 6.08) .. controls (4.76, 5.92) and (4.89, 5.75) .. (5.03, 5.59);
    \draw (5.03, 5.59) .. controls (5.15, 5.45) and (5.27, 5.31) .. (5.38, 5.17);
    \draw (5.38, 5.17) .. controls (5.53, 5.00) and (5.68, 4.82) .. (5.83, 4.64);
    \draw (5.83, 4.64) .. controls (6.06, 4.37) and (6.28, 4.10) .. (6.51, 3.83);
    \draw (6.64, 3.68) .. controls (6.75, 3.55) and (6.86, 3.42) .. (6.97, 3.29);
    \draw (7.09, 3.14) .. controls (7.20, 3.00) and (7.31, 2.87) .. (7.43, 2.74);
    \draw (7.55, 2.59) .. controls (7.62, 2.51) and (7.69, 2.43) .. (7.76, 2.34);
  \end{scope}
  \begin{scope}[color=linkcolor1]
    \draw (2.35, 3.01) .. controls (1.67, 4.26) and (0.82, 5.82) .. 
          (1.61, 6.44) .. controls (2.40, 7.07) and (3.17, 5.96) .. (3.84, 4.98);
    \draw (3.84, 4.98) .. controls (3.98, 4.78) and (4.11, 4.59) .. (4.24, 4.40);
    \draw (4.24, 4.40) .. controls (4.35, 4.24) and (4.45, 4.09) .. (4.56, 3.94);
    \draw (4.56, 3.94) .. controls (5.24, 2.94) and (6.03, 1.80) .. (6.49, 2.45);
    \draw (6.49, 2.45) .. controls (6.67, 2.70) and (6.85, 2.96) .. (7.03, 3.21);
    \draw (7.03, 3.21) .. controls (7.86, 4.39) and (8.76, 5.75) .. 
          (7.72, 6.39) .. controls (6.92, 6.88) and (6.03, 6.14) .. (5.44, 5.25);
    \draw (5.33, 5.09) .. controls (5.26, 4.99) and (5.19, 4.88) .. (5.12, 4.78);
    \draw (5.01, 4.62) .. controls (4.88, 4.42) and (4.75, 4.22) .. (4.61, 4.02);
    \draw (4.50, 3.85) .. controls (4.33, 3.58) and (4.15, 3.32) .. (3.97, 3.05);
    \draw (3.86, 2.88) .. controls (3.50, 2.34) and (2.73, 2.32) .. (2.45, 2.84);
  \end{scope}
  \begin{scope}[color=linkcolor2]
    \draw (2.71, 3.52) .. controls (2.25, 4.29) and (1.64, 5.33) .. 
          (1.99, 5.67) .. controls (2.33, 6.00) and (2.85, 5.00) .. (3.28, 4.18);
    \draw (3.28, 4.18) .. controls (3.40, 3.95) and (3.52, 3.71) .. (3.64, 3.48);
    \draw (3.64, 3.48) .. controls (3.73, 3.31) and (3.82, 3.14) .. (3.91, 2.96);
    \draw (3.91, 2.96) .. controls (4.23, 2.36) and (4.03, 1.64) .. 
          (3.48, 1.61) .. controls (2.89, 1.57) and (2.29, 1.77) .. (2.06, 2.30);
    \draw (1.99, 2.48) .. controls (1.31, 4.11) and (0.45, 6.16) .. 
          (1.40, 7.05) .. controls (2.28, 7.87) and (3.38, 6.72) .. (4.30, 5.62);
    \draw (4.30, 5.62) .. controls (4.44, 5.45) and (4.58, 5.29) .. (4.72, 5.12);
    \draw (4.72, 5.12) .. controls (4.84, 4.98) and (4.95, 4.84) .. (5.07, 4.70);
    \draw (5.07, 4.70) .. controls (5.21, 4.53) and (5.35, 4.36) .. (5.50, 4.19);
    \draw (5.50, 4.19) .. controls (5.84, 3.77) and (6.30, 3.42) .. (6.57, 3.75);
    \draw (6.57, 3.75) .. controls (7.07, 4.37) and (7.67, 5.11) .. 
          (7.21, 5.51) .. controls (6.78, 5.88) and (6.29, 5.28) .. (5.89, 4.72);
    \draw (5.77, 4.56) .. controls (5.70, 4.46) and (5.63, 4.37) .. (5.56, 4.27);
    \draw (5.44, 4.11) .. controls (5.33, 3.96) and (5.99, 3.10) .. (6.43, 2.53);
    \draw (6.55, 2.37) .. controls (6.77, 2.08) and (7.25, 2.25) .. (7.49, 2.66);
    \draw (7.49, 2.66) .. controls (8.43, 4.24) and (9.35, 6.08) .. 
          (8.02, 6.96) .. controls (7.03, 7.61) and (5.82, 6.79) .. (5.09, 5.67);
    \draw (4.98, 5.51) .. controls (4.91, 5.41) and (4.84, 5.30) .. (4.77, 5.20);
    \draw (4.66, 5.04) .. controls (4.54, 4.85) and (4.42, 4.66) .. (4.30, 4.48);
    \draw (4.19, 4.31) .. controls (4.02, 4.06) and (3.86, 3.82) .. (3.70, 3.57);
    \draw (3.59, 3.40) .. controls (3.39, 3.10) and (2.97, 3.07) .. (2.81, 3.35);
  \end{scope}
\end{tikzpicture}

